ScienceBenchmark: A Complex Real-World Benchmark for Evaluating Natural Language to SQL Systems

Natural Language to SQL systems (NL-to-SQL) have recently shown a significant increase in accuracy for natural language to SQL query translation. This improvement is due to the emergence of transformer-based language models, and the popularity of the Spider benchmark - the de-facto standard for evaluating NL-to-SQL systems. The top NL-to-SQL systems reach accuracies of up to 85\%. However, Spider mainly contains simple databases with few tables, columns, and entries, which does not reflect a realistic setting. Moreover, complex real-world databases with domain-specific content have little to no training data available in the form of NL/SQL-pairs leading to poor performance of existing NL-to-SQL systems. In this paper, we introduce ScienceBenchmark, a new complex NL-to-SQL benchmark for three real-world, highly domain-specific databases. For this new benchmark, SQL experts and domain experts created high-quality NL/SQL-pairs for each domain. To garner more data, we extended the small amount of human-generated data with synthetic data generated using GPT-3. We show that our benchmark is highly challenging, as the top performing systems on Spider achieve a very low performance on our benchmark. Thus, the challenge is many-fold: creating NL-to-SQL systems for highly complex domains with a small amount of hand-made training data augmented with synthetic data. To our knowledge, ScienceBenchmark is the first NL-to-SQL benchmark designed with complex real-world scientific databases, containing challenging training and test data carefully validated by domain experts.

==> tables/augment_1.tex <==
\begin{tabular}{l | l || l l l}
     Train Set & Eval Set& ValueNet & T5-Large w/o Picard & SmBoP+Grappa\\ \hline
     Spider Train (Zero-Shot)   & Spider Dev & 0.705 & 0.702 & 0.745 \\
     Spider Train+Synth Dev & Spider Dev  & 0.686 & 0.68 & 0.693 \\
     %Spider Train+Synth Dev Original  & Spider Dev &  & 0.879 & \\
     %Spider Train Synth  & Spider Dev &  &  & \\
     Spider Dev Synth  & Spider Dev & 0.403 &  0.369 & 0.683 \\
     \hline
\end{tabular}

==> tables/baseline_dbpal.tex <==
\begin{tabular}{l | r  r r r r}
     Train Set          & Spider    & CORDIS    & SDSS      & OncoMX   \\ \hline
     Spider Train       & 0.70      & 0.12      &  0.08     &  0.27      \\
      + Seed            & -         & 0.20      & 0.11      &  0.52      \\
      + DBPal           & 0.20*      & 0.24         & 0.07      &  0.37      \\
      + DBPal + Seed     & 0.68*      & 0.27         & 0.12      &  0.51     \\
      + Synth  (our approach)         & 0.40*      & 0.31      & 0.18      &  0.47     \\
      + Synth + Seed (our approach)    & 0.68*      & 0.35     & 0.21      &  0.57      \\
      \hline
      Improvement over DBPal & 0 &  \bf{+0.08}    & \bf{+0.09}      & \bf{+0.06}     & \bf{+0.11}  \\
     \hline
\end{tabular}

==> tables/database_stats.tex <==
\begin{tabular}[h]{@{} l r r r r r r @{}}

\toprule
     \textbf{Dataset} & \textbf{DBs} & \textbf{Tables }& \textbf{Columns} & \textbf{Rows} & \textbf{Avg Rows / Table} & \textbf{Size (GB})\\
\midrule
%     Spider & 186 & 641 (avg. 3.5) & 4,268 & 1,604,346 & 2,503 & 0.51 (avg 0.03)\\
     Spider & 186 & 641  & 4,268 & 1.6M & 2.5K & 0.51 \\
     (Avg / DB) & & 3.5 & 23 & 8.6K & & 0.03 \\
\midrule
\midrule
    \emph{ScienceBenchmark} & & & & & \\
\midrule
     CORDIS & 1 & 19 & 82 & 671K & 35K & 1 \\
     SDSS & 1 & 6 & 61 & 86M & 14M & 6.1 \\
     OncoMX & 1 & 25 & 106 & 65M & 2.6M & 12 \\ 
\bottomrule
\end{tabular}

==> tables/database_stats_rev.tex <==
\begin{tabular}[h]{@{} l r r r r r r r @{}}

\toprule
     \textbf{Dataset} & \textbf{DBs} & \textbf{Tables }& \textbf{Columns} & \textbf{Rows} & \textbf{Avg Rows / Table} & \textbf{Size (GB}) & \color{black}{\textbf{\#NL/SQL-pairs (manual+synth.)}}\\
\midrule
%     Spider & 186 & 641 (avg. 3.5) & 4,268 & 1,604,346 & 2,503 & 0.51 (avg 0.03)\\
     Spider & 186 & 641  & 4,268 & 1.6M & 2.5K & 0.51 & \color{black}{8,053 + 0}\\
     (Avg / DB) & & 3.5 & 23 & 8.6K & & 0.03 & \color{black}{43 + 0}\\
\midrule
     \color{black}{KaggleDBQA} & \color{black}{8} & \color{black}{17}  & \color{black}{179} & \color{black}{4.7M} & \color{black}{280K} & \color{black}{0.4} & \color{black}{272 + 0} \\
     \color{black}{(Avg / DB)} & & \color{black}{2.1} & \color{black}{22.3} & \color{black}{595K} & & \color{black}{0.05} & \color{black}{34 + 0}\\
\midrule
     \color{black}{
     BIRD} & \color{black}{81} & \color{black}{604}  & \color{black}{4,456} & \color{black}{3.7B} & \color{black}{608.8K} & \color{black}{33.4} & \color{black}{12,751 + 0} \\
     \color{black}{(Avg / DB)} & & \color{black}{7.5} & \color{black}{55} & \color{black}{4.5M} & & \color{black}{0.35} & \color{black}{135 + 0} \\
 % }
\midrule
\midrule
    \emph{ScienceBenchmark} & & & & & \\
\midrule
     CORDIS & 1 & 19 & 82 & 671K & 35K & 1 & \color{black}{200 + 1306}\\
     SDSS & 1 & 6 & 61 & 86M & 14M & 6.1 & \color{black}{200 + 2061}\\
     OncoMX & 1 & 25 & 106 & 65M & 2.6M & 12 & \color{black}{200 + 1065}\\ 
\bottomrule
\end{tabular}


==> tables/smbop_spec.tex <==
\begin{table}[!htbp]
%\centering
\small
\caption{Hyperparameters and hardware specifications for SmBoP in evaluation experiments}
\label{table:smbop_spec} 
\begin{tabular}{lc}
  \toprule
  \textbf{Hyperparameter}                  & \textbf{Selected Values}       \\ 
  \midrule
      Pretrained model & GraPPa-Large\\
      Dropout & 0.1 \\
      Learning rate base & 0.000186 \\
      Optimizer & Adam\\
      RAT Layers & 8 \\
      Beam Size & 30 \\
      Batch size & 16 \\
      Gradient Accum. & 4 \\
      Max sequence length & 512 \\
      Max steps & 60000 \\
      Early Stopping & 5 epochs \\
      \midrule
      \textbf{Hardware specifications}                  & \textbf{Values} \\
      \midrule
      CPU count & 8 \\
      GPU count & 1 \\
      GPU type &  nVidia T4 GPU \\
      Total running time of & \\ of all non-zeroshot experiments & \\
      in Table \ref{tab:augment2} & ca. 26 days\\
  \bottomrule
\end{tabular} 
\end{table}

==> tables/t5_spec.tex <==

\begin{table}[!htbp]
%\centering
\small
\caption{Hyperparameters and hardware specifications for T5-Large in evaluation experiments}
\label{table:t5_spec} 
\begin{tabular}{lc}
  \toprule
  \textbf{Hyperparameter}                  & \textbf{Selected Values}       \\ 
  \midrule
      Pretrained model & T5-Large\\
      Dropout & 0.1 \\
      Learning rate base & 0.0001 \\
      Optimizer & Adafactor\\
      Clip grad & 5 \\
      Accumulated iterations & 4 \\
      Batch size & 4 \\
      Gradient Accum. & 135 \\
      Max sequence length & 512 \\
      N\underline{o} of steps & 6500 \\
      \midrule
      \textbf{Hardware specifications}                  & \textbf{Values} \\
      \midrule
      CPU count & 8 \\
      GPU count & 1 \\
      GPU type & nVidia A100 GPU \\
      Total running time of & \\ all non-zeroshot experiments & \\
      in Table \ref{tab:augment2} & ca. 16 days\\
  \bottomrule
\end{tabular} 
\end{table}

==> tables/valuenet_spec.tex <==

\begin{table}[!htbp]
%\centering
\small
\caption{Hyperparameters and hardware specifications for ValueNet in evaluation experiments}
\label{table:valuenet_spec} 
% \catcode`,=\active
%\def,{\char`,\allowbreak}
%\renewcommand\arraystretch{1.2}
\begin{tabular}{lc}
  \toprule
  \textbf{Hyperparameter}                  & \textbf{Selected Values}       \\ 
  \midrule
      Pretrained model & \\
      of encoder & bart-base \\
      Seed & 90 \\
      Dropout & 0.3 \\
      Learning rate base & 0.001 \\
      Beam size & 1 \\
      Clip grad & 5 \\
      Accumulated iterations & 4 \\
      Batch size & 4 \\
      Column attention & affine \\
      N\underline{o} of epochs & 100 \\
      Hidden size & 300 \\
      Attention vector size & 300 \\ 
      Learning rate connection & 0.0001 \\
      Max grad norm & 1 \\
      Column embedding size & 300 \\
      Column poniter & true \\
      Learning rate of & \\
      Transformer & 2e-5 \\
      Max sequence length & 1024 \\
      Scheduler gamma & 0.5 \\
      Type embedding size & 128 \\
      Action embedding size & 128 \\
      Sketch loss weight & 1 \\ 
      Decode max time step & 80 \\
      Loss epoch threshold & 70 \\
      \midrule
      \textbf{Hardware specificcations}                  & \textbf{Values} \\
      \midrule
      CPU count & 8 \\
      GPU count & 1 \\
      GPU type & nVidia V100 GPU \\
      Total running time of & \\ all non-zeroshot experiments & \\
      in Table \ref{tab:augment2} & ca. 12 days\\
      %Total running time of & \\ 1 experiment & \\
      %in table \ref{tab:augment2} & ca. 1 day and 8 hours\\
      %Total running time of & \\ 1 experiment & \\
      %in table \ref{tab:augment2} & between 1 day 3 hours and 1 day 20 hours\\
  \bottomrule
\end{tabular} 
\end{table}

% below is the runtime of all experiments on ValueNet
\begin{comment}
{'_spider_original_oncomx_seed_synth_ursin_w_ga_4x4': 117709,
 '_spider_original_oncomx_synth_ursin_only_w_ga_4x4': 114206,
 '_spider_original_oncomx_seed_w_ga_4x4': 97164,
 '_spider_original_cordis_synth_ursin_seed_w_ga_4x4': 142283,
 '_spider_original_cordis_synth_ursin_only_w_ga_4x4': 110572,
 '_spider_original_sdss_synth_only_w_ga_4x4': 154518,
 '_spider_original_sdss_seed_synth_w_ga_4x4': 111668,
 '_spider_original_sdss_seed_w_ga_4x4': 99020,
 '_spider_original_cordis_seed_w_ga_4x4': 100409,}
total : 1047549 (seconds) 12 days 2 hours 59 min 9 sec
\end{comment}
